Enhancing naive classifier for positive unlabeled data based on logistic regression approach

We argue that for analysis of Positive Unlabeled (PU) data under Selected Completely At Random (SCAR) assumption it is fruitful to view the problem as fitting of misspecified model to the data. Namely, we show that the results on misspecified fit imply that in the case when posterior probability of the response is modelled by logistic regression, fitting the logistic regression to the observable PU data which {\it does not} follow this model, still yields the vector of estimated parameters approximately colinear with the true vector of parameters. This observation together with choosing the intercept of the classifier based on optimisation of analogue of F1 measure yields a classifier which performs on par or better than its competitors on several real data sets considered.

==> References_ENH.tex <==
@InProceedings{PUICCS,
    author="Teisseyre, P.
        and Mielniczuk, J. and {\L}az{e}cka, M ",
   title="Different strategies of fitting logistic regression for positive and unlabeled data",
    booktitle="Proceedings of the International Conference on Computational Science ICCS'20",
    year="2020",
    publisher="Springer International Publishing",
    address="Cham",
    pages="3--17"
   }




@article{LBE,
    title={Instance-Dependent Positive and Unlabeled Learning with Labeling Bias Estimation},
    author={Chen Gong and Qizhou Wang and Tongliang Liu and Bo Han and Jane Jia You and Jian Yang and Dacheng Tao},
    journal={IEEE transactions on pattern analysis and machine intelligence},
    year={2021},
    volume={PP}
}
@article{Ruud,
    title={Sufficient conditions for the consistency of maximum likelihood estimation despite misspecification of distribution in multinomial  discrete choice models},
    author={Ruud, P.},
    journal={Econometrica},
    year={1983},
    volume={51},
    pages=225-228
}

@article{Vuong,
    title={Likelihood ratio tests for model selection and non-nested hypotheses},
    author={Vuong, Q.},
    journal={Econometrica},
    year={1989},
    volume={57},
    pages= 307-333
}



@inproceedings{GerychPropensity,
    title={Recovering The Propensity Score From Biased Positive Unlabeled Data},
    author={Walter Gerych and Thomas Hartvigsen and Luke Buquicchioand Emmanuel Agu and Elke Rundensteiner},
    booktitle={AAAI},
    year={2022}
}

@inproceedings{Tabata2020,
    title={Estimating the {F}1 score for learning from positive and unlabeled examples},
    author={Tabatabaei, S. and Klein, J. and Hoogendoorn, M},
    booktitle={LOD 2020},
    publisher={Springer, Cham},
    year={2020}
}



@inproceedings{IIC,
    title={Invariant information clustering for unsupervised image classification and segmentation},
    author={Ji, Xu and Henriques, Jo{\~a}o F and Vedaldi, Andrea},
    booktitle={Proceedings of the IEEE International Conference on Computer Vision},
    pages={9865--9874},
    year={2019}
}

@inproceedings{VaDE,
    title={Variational Deep Embedding: An Unsupervised and Generative Approach to Clustering},
    author={Zhuxi Jiang and Yin Zheng and Huachun Tan and Bangsheng Tang and Hanning Zhou},
    booktitle={IJCAI},
    year={2017}
}

@inproceedings{ConformalInferenceVovk,
    author = {Vovk, Volodya and Gammerman, Alexander and Saunders, Craig},
    title = {Machine-Learning Applications of Algorithmic Randomness},
    year = {1999},
    month = jun,
    isbn = {1558606122},
    publisher = {Morgan Kaufmann Publishers Inc.},
    address = {San Francisco, CA, USA},
    booktitle = {Proceedings of the Sixteenth International Conference on Machine Learning},
    pages = {444453},
    numpages = {10},
    series = {ICML '99}
}

@inproceedings{LeeLiu03,
    author = {Lee, W. and Liu, B.},
    title = {Learning with positive and unlabeled exampled using weighted logistic regression},
    year = {2003},
   publisher = {Morgan Kaufmann Publishers Inc.},
    address = {San Francisco, CA, USA},
    booktitle = {Proceedings of the Twentieth International Conference on Machine Learning},
    pages = {448-455},
     series = {ICML '03}
}

%%


@inbook{ConformalInferenceVovk2,
    author = {Vovk, Vladimir and Gammerman, Alex and Shafer, Glenn},
    year = {2005},
    month = jan,
    pages = {},
    title = {Algorithmic Learning in a Random World},
    journal = {Algorithmic Learning in a Random World},
    note = {DOI: 10.1007/b106715},
    publisher = {Springer Science \& Business Media},
    address = {New York, NY}
}

@inproceedings{NaVAE,
    author = {Na, Byeonghu and Kim, Hyemi and Song, Kyungwoo and Joo, Weonyoung and Kim, Yoon-Yeong and Moon, Il-Chul},
    title = {Deep Generative Positive-Unlabeled Learning under Selection Bias},
    year = {2020},
    isbn = {9781450368599},
    publisher = {Association for Computing Machinery},
    address = {New York, NY, USA},
    note = {DOI: 10.1145/3340531.3411971},
    doi = {10.1145/3340531.3411971},
    booktitle = {Proceedings of the 29th ACM International Conference on Information \& Knowledge Management},
    pages = {1155-1164},
    numpages = {10},
    keywords = {positive-unlabeled learning, selection bias, variational autoencoders},
    location = {Virtual Event, Ireland},
    series = {CIKM '20}
}

@misc{ConformalPValues,
    title={Testing for Outliers with Conformal p-values}, 
    author={Stephen Bates and Emmanuel Candes and Lihua Lei and Yaniv Romano and Matteo Sesia},
    year={2021},
    eprint={2104.08279},
    archivePrefix={arXiv},
    primaryClass={stat.ME}
}

@inproceedings{TeisseyreAISTATCHANGE!!!,
    title={Joint estimation of posterior probability and propensity score function for positive and unlabelled data}, 
    author={Teisseyre, P. and Lazecka, M. and Mielniczuk, J.},
    year={2021},
    booktitle={AISTAT 2021 (preprint)}
}

@inproceedings{SVMPenaltyKe,
    author = {Ke, T. and Yang, B. and Zhen, L. and Tan, J. and Li, Y. and Jing, L.},
    year = {2012},
    title = {Building high-performance classifiers using positive and unlabeled examples for text classification},
    booktitle = {International Symposium on Neural Networks},
    publisher = {Springer},
    pages = {187--195},
}

@InProceedings{SVMWeights,
    author="Liu, Zhigang
    and Shi, Wenzhong
    and Li, Deren
    and Qin, Qianqing",
    editor="Li, Xue
    and Wang, Shuliang
    and Dong, Zhao Yang",
    title={Partially supervised classification -- based on weighted unlabeled samples support vector machine},
    booktitle="Advanced Data Mining and Applications",
    year="2005",
    publisher="Springer Berlin Heidelberg",
    address="Berlin, Heidelberg",
    pages="118--129"
}

@inproceedings{WeightedLogReg,
    author = {Lee, W.S. and Liu, B.},
    year = {2003},
    title = {Learning with positive and unlabeled examples using weighted logistic regression},
    booktitle = {Proceedings of the Twentieth International Conference on Machine Learning},
    pages = {448-455},
}

@INPROCEEDINGS{WeightedElkan,
    author = {Charles Elkan},
    title = {The foundations of cost-sensitive learning},
    booktitle = {In Proceedings of the Seventeenth International Joint Conference on Artificial Intelligence},
    year = {2001},
    pages = {973--978}
}

@INPROCEEDINGS{DCCP,
    author = {Xinyue Shen and Steven Diamond and Yuantao Gu and Stephen Boyd},
    title = {Disciplined Convex-Concave Programming},
    booktitle = {In Proceedings of 2016 IEEE 55th Conference on Decision and Control (CDC)},
    year = {2016},
    pages = {1009--1014},
    note = {DOI: 10.1109/CDC.2016.7798400}
}

@inproceedings{bekker2019ecml,
    author = {Bekker, J. and Robberechts, P. and Davis, J.},
    title = {Beyond the selected completely at random assumption for learning from positive and unlabeled data},
    booktitle = {{P}roceedings of the 2019 {E}uropean {C}onference on {M}achine {L}earning and {P}rinciples and {P}ractice of {K}nowledge {D}iscovery in {D}atabases},
    editor = {Brefeld, Ulf and Fromont, {\'E}lisa and Hotho, Andreas and Knobbe, Arno J. and Maathuis, Marloes H. and Robardet, C{\'e}line},
    publisher = {Springer, Cham},
    pages = {71--85},
    year = {2019},
    note = {DOI: 10.1007/978-3-030-46147-8\_5},
    isbn = {978-3-030-46147-8}
}

@inproceedings{Liu2003,
    author = {Liu, B. and Dai, Y. and Li, X. and Lee, W. S. and Yu, P. S.},
    title = {Building Text Classifiers Using Positive and Unlabeled Examples},
    booktitle = {Proceedings of the Third IEEE International Conference on Data Mining},
    series = {ICDM '03},
    year = {2003},
    pages={179--186},
    note={DOI: 10.1109/ICDM.2003.1250918}
} 

@InProceedings{DCPGraphImpl,
    author="Grant, Michael C.
        and Boyd, Stephen P.",
    editor="Blondel, Vincent D.
        and Boyd, Stephen P.
        and Kimura, Hidenori",
    title={Graph implementations for nonsmooth convex programs},
    booktitle="Recent Advances in Learning and Control",
    year="2008",
    publisher="Springer London",
    address="London",
    pages="95--110"
}

@inproceedings{ElkanNoto,
    author = {Elkan, C. and Noto, K.},
    year = {2008},
    month = aug,
    pages = {213--220},
    title = {Learning classifiers from only positive and unlabeled data},
    booktitle = {Proceedings of the ACM SIGKDD International Conference on Knowledge Discovery and Data Mining},
    note = {DOI: 10.1145/1401890.1401920}
}

@INPROCEEDINGS{SVMPenaltyLiu,
    author={Liu, B. and Dai, Y. and Li, X. and Lee, W.S. and Yu, P.S.},
    booktitle={Third IEEE International Conference on Data Mining}, 
    title={Building text classifiers using positive and unlabeled examples}, 
    year={2003},
    pages={179--186},
    note={DOI: 10.1109/ICDM.2003.1250918}
}

@article{TIcE,
    title={Estimating the class prior in positive and unlabeled data through decision tree induction}, volume={32}, 
    url={https://ojs.aaai.org/index.php/AAAI/article/view/11715},
    number={1},
    journal={Proceedings of the AAAI Conference on Artificial Intelligence},
    author={Bekker, Jessa and Davis, Jesse},
    year={2018},
    pages={2712--2719},
    month=apr
}

@article{AMCS,
    title={Strategies for fitting logistic regression for positive and unlabeled data revisited}, 
journal={Int.J. Appl. Math. Comp. Sci.},
    author={Wawrzenczyk, A. and Mielniczuk, J.},
    year={2022},
    pages={299-309},
   
}


@article{LiDuan,
author = {Li, K-C. and Duan, N.},
title = {Regression  analysis under link violation},
volume = {17},
journal = {The Annals of Statistics},
number = {3},
publisher = {Institute of Mathematical Statistics},
pages = {1009--1052},
year = {1989},

}

@article{Fowlkes,
author = {Fowlkes, E. and Mallows, C.},
title = {A method for comparing two hierarchical clusterings},
volume = {78},
journal = {Journal of American Statistical Association},
pages = {573-586},
year = {1981},

}

@article{White1982,
author = {White, H.},
title = {Maximum likelihood estimation of misspecified models},
volume = {50},
journal = {Econometrica},
number = {1},
pages = {1-25},
year = {1982},

}




@Article{MM2021,
    author={{\L}az{e}cka, M.
        and Mielniczuk, J.     and Teisseyre, P.},
    title={Estimating the class prior for positive and unlabelled data via logistic regression},
    journal={Advances in Data Analysis and Classification},
    year={2021},
    pages={1039--1068},
    month=jun,
    day={3},
    volume={15},
    number={4},
    note={DOI: 10.1007/s11634-021-00444-9}
}

@article{Bahorik2014,
    title={Under-reporting of drug use among individuals with schizophrenia: prevalence and predictors},
    author={Bahorik, A. L.
        and Newhill, C. E.
        and Queen, C. C.
        and Eack, S. M.},
    journal={Psychological Medicine},
    year={2014},
    volume={44},
    number={12},
    pages={
          61--69
        },
    note={DOI: 10.1017/S0033291713000548}
}

@article{Yang2014,
    title={Ensemble positive unlabeled learning for disease gene identification},
    author={P. Yang and X. Li and H. Chua and C. Kwoh and S. Ng},
    journal={PLOS ONE},
    year={2014},
    volume={9},
    number={5},
    pages={1--11},
    note={DOI: 10.1371/journal.pone.0097079}
}

@article{Ward2009,
    title={Presence-only data and the {EM} algorithm},
    author={G. Ward and T. Hastie and S. Barry and J. Elith and J. Leathwick},
    journal={Biometrics},
    year={2009},
    volume={65},
    pages={554--563},
    note={DOI: 10.1111/j.1541-0420.2008.01116.x}
}

@article{CCCP,
    author = {Yuille, Alan and Rangarajan, Anand},
    year = {2003},
    month = apr,
    pages = {915--936},
    title = {The concave-convex procedure},
    volume = {15},
    number = {4},
    journal = {Neural Computation},
    note = {DOI: 10.1162/08997660360581958}
}

@article{BekkerSurvey,
   title={Learning from positive and unlabeled data: a survey},
   volume={109},
   number={4},
   journal={Machine Learning},
   publisher={Springer Science and Business Media LLC},
   author={Bekker, J. and Davis, J.},
   year={2020},
   month=apr,
   pages={719-760},
   note={DOI: 10.1007/s10994-020-05877-5}
}

@article{SECHIDIS2017,
    title = "Dealing with under-reported variables: An information theoretic solution",
    journal = "International Journal of Approximate Reasoning",
    volume = "85",
    number = "1",
    pages = "159--177",
    year = "2017",
    author = "Sechidis, K. and Sperrin, M. and Petherick, E. S. and  Luján, M. and  Brown, G.",
    note = {DOI: 10.1016/j.ijar.2017.04.002}
}

@article{SVMBagging,
    author = {Mordelet, Fantine and Vert, Jean-Philippe},
    year = {2010},
    month = oct,
    pages = "201--209",
    title = {A bagging {SVM} to learn from positive and unlabeled examples},
    volume = {37},
    number = {1},
    journal = "Pattern Recognition Letters",
    note = {DOI: 10.1016/j.patrec.2013.06.010}
}

@article{SVMBootstrap,
   title={A robust ensemble approach to learn from positive and unlabeled data using {SVM} base models},
   volume={160},
   journal={Neurocomputing},
   publisher={Elsevier BV},
   author={Claesen, Marc and De Smet, Frank and Suykens, Johan A.K. and De Moor, Bart},
   year={2015},
   month=jul,
   pages={73-84},
   note={DOI: 10.1016/j.neucom.2014.10.081}
}

@article{LippBoyd2016,
    author={Thomas Lipp and Steven Boyd},
    title={Variations and extension of the convex-concave procedure},
    journal={Optimisation and Engineering},
    year={2016},
    volume={17},
    number={2},
    pages={263--287},
    note={DOI: 10.1007/s11081-015-9294-x}
}

@article{DCPConeProgram,
    author = { Yu.   Nesterov  and    A.   Nemirovsky },
    title = {Conic formulation of a convex programming problem and duality},
    journal = {Optimization Methods and Software},
    volume = {1},
    number = {2},
    pages = {95--115},
    year  = {1992},
    publisher = {Taylor \& Francis},
    note = {DOI: 10.1080/10556789208805510}
}

@InProceedings{ADGAN,
author="Schlegl, Thomas
and Seeb{\"o}ck, Philipp
and Waldstein, Sebastian M.
and Schmidt-Erfurth, Ursula
and Langs, Georg",
editor="Niethammer, Marc
and Styner, Martin
and Aylward, Stephen
and Zhu, Hongtu
and Oguz, Ipek
and Yap, Pew-Thian
and Shen, Dinggang",
title="Unsupervised Anomaly Detection with Generative Adversarial Networks to Guide Marker Discovery",
booktitle="Information Processing in Medical Imaging",
year="2017",
publisher="Springer",
pages="146--157",
}


@article{BFGSFail,
    author = {Mascarenhas, Walter},
    year = {2004},
    month = jan,
    pages = {49--61},
    title = {The BFGS method with exact line searches fails for non-convex objective functions},
    volume = {99},
    journal = {Mathematical Programming},
    note = {DOI: 10.1007/s10107-003-0421-7}
}

@article{Heckman,
    author = {Heckman, J.},
    journal = {Econometrica},
     pages = {153-161},
    title = {Sample selection bias as a specification error},
    volume = {47},
    year = {1979}
}

@article{Schnabel, 
title={Recommendation as treatments: debiasing learning and evaluation},
journal={ICML}, 
volume={48},
author={Shnabel, Thobias and Swaminathan, Adith and  Singh, Ashudeep and  Chandak, Navin and Joachims, Thorsten}, 
year={2016}, 
pages={1670-1679} 
}




@article{Storey,
    author = {Storey,J.},
    journal = {Journal of the Royal Statistical Society. Series B (Methodological)},
     pages = {479-498},
    publisher = {[Royal Statistical Society, Wiley]},
    title = {Direct approach to false discovery rates},
    volume = {64},
    year = {2002}
}

@article{EM,
    author = {A. P. Dempster and N. M. Laird and D. B. Rubin},
    journal = {Journal of the Royal Statistical Society. Series B (Methodological)},
    number = {1},
    pages = {1--38},
    publisher = {[Royal Statistical Society, Wiley]},
    title = {Maximum likelihood from incomplete data via the {EM} algorithm},
    volume = {39},
    year = {1977},
    note = {DOI: 10.1111/j.2517-6161.1977.tb01600.x}
}

@book{DCP,
    author="Grant, Michael
        and Boyd, Stephen
        and Ye, Yinyu",
    editor="Liberti, Leo
        and Maculan, Nelson",
    title="Disciplined convex programming",
    bookTitle={Global Optimization: From Theory to Implementation"},
    year="2006",
    publisher="Springer US",
    address="Boston, MA",
    pages="155--210",
    note={DOI: 10.1007/0-387-30528-9_7}
}
@article{Jain,
author = {Jain, Shantanu and Delano, Justin and Sharma, Himanshu and Radivojac, Predrag},
year = {2020},
month = {04},
pages = {4255-4263},
title = {Class Prior Estimation with Biased Positives and Unlabeled Examples},
volume = {34},
journal = {Proceedings of the AAAI Conference on Artificial Intelligence}
}



@inproceedings{nnPU,
    title={Learning from Positive and Unlabeled Data with a Selection Bias},
    author={Masahiro Kato and Takeshi Teshima and Junya Honda},
    booktitle={International Conference on Learning Representations},
    year={2019}
}

@INPROCEEDINGS{ECOD,
    author = {Li, Zheng and Zhao, Yue and Hu, Xiyang and Botta, Nicola and Ionescu, Cezar and Chen, George H.},
    title = {ECOD: Unsupervised Outlier Detection Using Empirical Cumulative Distribution Functions},
    booktitle = {IEEE Transactions on Knowledge and Data Engineering},
    year = {2022},
    note = {DOI: 10.1109/TKDE.2022.3159580}
}

@article{OCCOverview,
    author = {Ruff, L. and Kauffmann, J. and Vandermeulen, R. and Montavon, G. and Samek, W. and Kloft, M. and Dietterich, T. and Müller, K.},
    year = {2021},
    month = feb,
    pages = {1--40},
    title = {A Unifying Review of Deep and Shallow Anomaly Detection},
    volume = {PP},
    journal = {Proceedings of the IEEE}
}

@article{OCCDefinition1,
       author = {{Moya}, M.~M. and {Koch}, M.~W. and {Hostetler}, L.~D.},
        title = "{One-class classifier networks for target recognition applications}",
         year = 1993,
        month = jan,
        pages = {24043},
      journal = {NASA STI/Recon Technical Report},
       volume = {N 93},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1993STIN...9324043M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{OCCDefinition2,
    title = {A review of novelty detection},
    journal = {Signal Processing},
    volume = {99},
    pages = {215--249},
    year = {2014},
    issn = {0165-1684},
    note = {DOI: 10.1016/j.sigpro.2013.12.026},
    author = {Marco A.F. Pimentel and David A. Clifton and Lei Clifton and Lionel Tarassenko},
}

@book{CoverThomas,
    author={Cover, T. and J. Thomas},
    title={Elements of Information Theory},
    year={1991},
    address="New York, NY",
    publisher={Wiley},
    note={DOI: 10.1002/047174882X}
}

@book{Bishop,
    author={Bishop, Ch.},
    title={Pattern Recognition and Machine Learning},
    year={2006},
    address="New York, NY",
    publisher={Springer}
    
}
@book{MM_source,
    author = {Hastie, Trevor and Tibshirani, Robert and Wainwright, Martin},
    year = {2015},
    month = may,
    pages = {1--337},
    isbn = {9780429171581},
    title = {Statistical Learning with Sparsity: The Lasso and Generalizations},
    publisher = {Chapman and Hall/CRC},
    note = {DOI: 10.1201/b18401}
}

@INPROCEEDINGS{COPOD,
    author={Li, Zheng and Zhao, Yue and Botta, Nicola and Ionescu, Cezar and Hu, Xiyang},
    booktitle={2020 IEEE International Conference on Data Mining (ICDM)}, 
    title={COPOD: Copula-Based Outlier Detection}, 
    year={2020},
    volume={},
    number={},
    pages={1118--1123},
    note = {DOI: 10.1109/ICDM50108.2020.00135},
}

@incollection{A^3,
	year = 2021,
	publisher = {Springer International Publishing},
	pages = {69--84},
	author = {Philip Sperl and Jan-Philipp Schulze and Konstantin Böttinger},
	title = {Activation Anomaly Analysis},
	booktitle = {Machine Learning and Knowledge Discovery in Databases},
    note = {DOI: 10.1007/978-3-030-67661-2\_5},
}

@INPROCEEDINGS{IForest,
    author={Liu, Fei Tony and Ting, Kai Ming and Zhou, Zhi-Hua},
    booktitle={2008 Eighth IEEE International Conference on Data Mining}, 
    title={Isolation Forest}, 
    year={2008},
    volume={},
    number={},
    pages={413--422},
    note = {DOI: 10.1109/ICDM.2008.17},
}

@article{OC-SVM,
    author = {Schölkopf, Bernhard and Platt, John and Shawe-Taylor, John and Smola, Alexander and Williamson, Robert},
    year = {2001},
    month = jul,
    pages = {1443--1471},
    title = {Estimating Support of a High-Dimensional Distribution},
    volume = {13},
    journal = {Neural Computation},
    note = {DOI: 10.1162/089976601750264965},
}

@inproceedings{PUSB,
    author = {Kiryo, Ryuichi and Niu, Gang and du Plessis, Marthinus C. and Sugiyama, Masashi},
    title = {Positive-Unlabeled Learning with Non-Negative Risk Estimator},
    year = {2017},
    isbn = {9781510860964},
    publisher = {Curran Associates Inc.},
    address = {Red Hook, NY, USA},
    booktitle = {Proceedings of the 31st International Conference on Neural Information Processing Systems},
    pages = {1674-1684},
    numpages = {11},
    location = {Long Beach, California, USA},
    series = {NIPS'17}
}
